Improving Knowledge Graph Representation Learning by Structure Contextual Pre-training

Representation learning models for Knowledge Graphs (KG) have proven to be effective in encoding structural information and performing reasoning over KGs. In this paper, we propose a novel pre-training-then-fine-tuning framework for knowledge graph representation learning, in which a KG model is firstly pre-trained with triple classification task, followed by discriminative fine-tuning on specific downstream tasks such as entity type prediction and entity alignment. Drawing on the general ideas of learning deep contextualized word representations in typical pre-trained language models, we propose SCoP to learn pre-trained KG representations with structural and contextual triples of the target triple encoded. Experimental results demonstrate that fine-tuning SCoP not only outperforms results of baselines on a portfolio of downstream tasks but also avoids tedious task-specific model design and parameter training.

==> tables/dataset-pretraining.tex <==
\begin{table}\footnotesize%
\centering
% \fontsize{8pt}{24pt}
\renewcommand\arraystretch{1.2}
\begin{tabular}{lccccc}
\toprule
\textbf{Dataset}  & \textbf{\# Ent} & \textbf{\# Rel} &
\textbf{\# Triples} \\
\midrule
% WN11     & 38,696 &    11 & 125,734 \\
% WN18     & 40,943 &    18 & 151,442 \\
% WN18RR   & 40,943 &    11 &  93,003 \\
WN-all   & 116,377 & 26 & 377,592  \\
% \midrule
% noun  &  82,115 & 19 & 269,261 \\
% verb  &  13,710 & 11 &  54,947 \\
% adj   &  18,151 &  9 &  49,341\\
% adv   &   2,671 &  5 &  4,043 \\
\bottomrule
\end{tabular}
\caption{\label{tab:dataset-WordNet-all} Datasets for pre-training.}
\end{table}

==> tables/entity-alignment-and-typing.tex <==

\begin{table*}[tp]
  \centering
%  \fontsize{6.5}{8}\selectfont
%   \begin{threeparttable}
  \label{tab:performance_comparison}
  {\tabcolsep0.13in
  \small
    \begin{tabular}{lcccccccc}
    \toprule
    \multirow{2}{*}{\textbf{Method}}&
    \multicolumn{4}{c}{\textbf{Entity Alignment}}&\multicolumn{4}{c}{\textbf{Entity Typing}}\cr
    \cmidrule(lr){2-5} \cmidrule(lr){6-9}
    & MRR & Hit@1 & Hit@3 & Hit@10 & MRR & Hit@1 & Hit@3 & Hit@10\cr
    \midrule
    TransE
    	& 0.2973 & 0.00 & 41.07 & 67.85 & 0.0083 & 0.47 & 1.27 & 2.31 \cr
	DistMult
	 	& 0.3294 & 14.28 & 42.85 & 64.28 & 0.0387 & 1.67 & 3.59 & 8.31 \cr
	ComplEx
		& 0.3424 & 18.75 & 45.53 & 62.50 & 0.0294 & 1.43 & 3.19 & 5.43 \cr
    HolE
    	& 0.2779 & 13.39 & 39.28 & 61.60 & 0.0216 & 0.31 & 0.47 & 0.56 \cr
%     HypER
%     	& & & & & & & & \cr
%     TuckER
%     	& & & & & & & & \cr
%     InteractE
%     	& & & & & & & & \cr
%     Decom
%     	& & & & & & & & \cr
%     DihEdral
%     	& & & & & & & & \cr
%    KBAT \citep{KBAT-Nathani-2019}
%    	& 0.441  & 0.361  & 0.483  & 0.581  & 0.518  & 0.46   & 0.54   & 0.626  \cr
    % RotatE
    % 	& & & & & & & & \cr
    \midrule
    SCoP & 0.8485 & 83.92 & 85.71 & 85.71 & 0.4570 & 44.40 & 44.56 & 44.64 \cr
    \bottomrule
   \end{tabular}
   }
%   \end{threeparttable}
\caption{\label{tab:link-prediction}
% Link prediction results on WN18RR and FB15k-237 with pre-trained SCoP.
Link prediction results. The bold numbers are the best one among all results.
}
\end{table*}

==> tables/extreme-relation-link-prediction.tex <==
% \begin{table*}[tp]
%   \centering
% %  \fontsize{6.5}{8}\selectfont
%   \begin{threeparttable}
%   \label{tab:performance_comparison}
%   {\tabcolsep0.13in
% %   \small
%     \begin{tabular}{lcccccccc}
%     \toprule
%     \multirow{2}{*}{\textbf{Dataset}}&
%     \multicolumn{2}{c}{\textbf{rel-1}}&\multicolumn{2}{c}{\textbf{rel-2}}&\multicolumn{2}{c}{\textbf{rel-3}}&\multicolumn{2}{c}{\textbf{rel-4}}\cr
%     \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
%     & MRR & Hit@1 & MRR & Hit@1 & MRR & Hit@1 & MRR & Hit@1 \cr
%     \midrule
%     TransE
%     	& & & & & & & &\cr
% 	DistMult
% 	 	& & & & & & & &\cr
% 	ComplEx
% 		& & & & & & & & \cr
%     % HolE
%     % 	& 0.2779 & 13.39 & 39.28 & 61.60 & 0.0216 & 0.31 & 0.47 & 0.56 \cr
% %     HypER
% %     	& & & & & & & & \cr
% %     TuckER
% %     	& & & & & & & & \cr
% %     InteractE
% %     	& & & & & & & & \cr
% %     Decom
% %     	& & & & & & & & \cr
% %     DihEdral
% %     	& & & & & & & & \cr
% %    KBAT \citep{KBAT-Nathani-2019}
% %    	& 0.441  & 0.361  & 0.483  & 0.581  & 0.518  & 0.46   & 0.54   & 0.626  \cr
%     % RotatE
%     % 	& & & & & & & & \cr
%     \midrule
%     SCoP & & & & & & & &  \cr
%     \bottomrule
%   \end{tabular}
%   }
%   \end{threeparttable}

% \end{table*}

\begin{table*}[tp]
  \centering
%  \fontsize{6.5}{8}\selectfont
%   \begin{threeparttable}
  \label{tab:performance_comparison}
  {\tabcolsep0.13in
%   \small
    \begin{tabular}{lccccccc}
    \toprule
    Method & WN-7k & WN-5k & WN-7t & WN-5t & WN-3h & WN-1h & avarage \cr
    % \multirow{2}{*}{\textbf{Method}}&
    % \multicolumn{2}{c}{\textbf{rel-5}}&\multicolumn{2}{c}{\textbf{rel-6}}&\multicolumn{2}{c}{\textbf{rel-7}}&\multicolumn{2}{c}{\textbf{avarage}}\cr
    % \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
    % & MRR & Hit@1 & MRR & Hit@1 & MRR & Hit@1 & MRR & Hit@1 \cr
    \midrule
    TransE
    	& & & 26.43 & & & &\cr
	DistMult
	 	& & & & & & &\cr
	ComplEx
		& & & & & & & \cr
    % HolE
    % 	& 0.2779 & 13.39 & 39.28 & 61.60 & 0.0216 & 0.31 & 0.47 & 0.56 \cr
%     HypER
%     	& & & & & & & & \cr
%     TuckER
%     	& & & & & & & & \cr
%     InteractE
%     	& & & & & & & & \cr
%     Decom
%     	& & & & & & & & \cr
%     DihEdral
%     	& & & & & & & & \cr
%    KBAT \citep{KBAT-Nathani-2019}
%    	& 0.441  & 0.361  & 0.483  & 0.581  & 0.518  & 0.46   & 0.54   & 0.626  \cr
    % RotatE
    % 	& & & & & & & & \cr
    \midrule
    SCoP & 67.54 & 86.58 & 78.51 & 62.10 & 40.81 & 19.04 &  \cr
    \bottomrule
   \end{tabular}
   }
%   \end{threeparttable}
\caption{\label{tab:link-prediction}
% Link prediction results on WN18RR and FB15k-237 with pre-trained SCoP.
Hit@1 results of link prediction on different fine-tuning dataset. The bold numbers are the best one among all results.
}
\end{table*}

==> tables/threshold-triple-classification.tex <==
\begin{table}\footnotesize%
\centering
% \fontsize{8pt}{24pt}
\renewcommand\arraystretch{1.2}
\begin{tabular}{lccccc}
\toprule
\textbf{Dataset}  & \textbf{\# TransE} &
\textbf{\# Train} & \textbf{\# Dev} & \textbf{\# Test} \\
\midrule
% \hline
%WN18     & 40,943 &    18 & 141,442 &  5,000 &  5,000 \\
% WordNet-all & 116,377 &  302,074 &  37,759 &  37,759 \\
%FB15K    & 14,951 & 1,345 & 383,142 & 50,000 & 59,071 \\
% FB15k-237 & 14,541 &   237 & 272,115 & 17,535 & 20,466 \\
E-Typing    & 87,875 &  72,076 & 8,431 & 8,582 \\
E-Alignment & 13,205 &  17,725 & 1,805 & 1,856 \\
% \midrule
% WN-7k-r3  & 87,875 &  72,105 & 8,552 & 8,432 \\
% WN-5k-r12 & 36,097 &  58,161 & 8,214 & 8,342 \\
% WN-7t-r7  & 10,197 &   7,066 & 1,021 & 1010 \\
% WN-5t-r13 &  6,823 &   5,125 &   808 & 702 \\
% WN-3h-r19 &    647 &     320 &    38 & 49 \\
% WN-1h-r20 &    417 &     170 &    29 & 21 \\
\bottomrule
\end{tabular}
\caption{\label{tab:dataset} Dataset for fine-tuning.}
\end{table}
